AST-Probe: Recovering abstract syntax trees from hidden representations of pre-trained language models

The objective of pre-trained language models is to learn contextual representations of textual data. Pre-trained language models have become mainstream in natural language processing and code modeling. Using probes, a technique to study the linguistic properties of hidden vector spaces, previous works have shown that these pre-trained language models encode simple linguistic properties in their hidden representations. However, none of the previous work assessed whether these models encode the whole grammatical structure of a programming language. In this paper, we prove the existence of a syntactic subspace, lying in the hidden representations of pre-trained language models, which contain the syntactic information of the programming language. We show that this subspace can be extracted from the models' representations and define a novel probing method, the AST-Probe, that enables recovering the whole abstract syntax tree (AST) of an input code snippet. In our experimentations, we show that this syntactic subspace exists in five state-of-the-art pre-trained language models. In addition, we highlight that the middle layers of the models are the ones that encode most of the AST information. Finally, we estimate the optimal size of this syntactic subspace and show that its dimension is substantially lower than those of the models' representation spaces. This suggests that pre-trained language models use a small part of their representation spaces to encode syntactic information of the programming languages.

==> random.tex <==
\begin{table*}
\caption{UAS scores -- Python}
\begin{center}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{.5pt}
    
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{13}{l|cccccccccccc}}
    \toprule
        \multicolumn{1}{l}{} &
        \multicolumn{12}{c}{\textbf{Test UAS}} \\
        \cline{2-13}
        
     \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{L--1} & \multicolumn{1}{c}{L--2} & \multicolumn{1}{c}{L--3} & \multicolumn{1}{c}{L--4} & \multicolumn{1}{c}{L--5} & \multicolumn{1}{c}{L--6} & \multicolumn{1}{c}{L--7} & \multicolumn{1}{c}{L--8} & \multicolumn{1}{c}{L--9} & \multicolumn{1}{c}{L--10} & \multicolumn{1}{c}{L--11} & \multicolumn{1}{c}{L--12} \\ 
        
    \midrule
        CodeBERT-base-baseline & & & & & & & & & & & & \\
        
    \midrule
        CodeBERT-base & & & & & & & & & & & & \\
        
        CodeBERTa-small & & & & & & & & & & & & \\
        
        RoBERTa (NLP) & & & & & & & & & & & & \\
    
        GraphCodeBERT & & & & & & & & & & & & \\

        CodeT5 & & & & & & & & & & & & \\
    \bottomrule
    \end{tabular*}
\end{center}

\label{tab:models}
\end{table*}


\begin{table}[]
\begin{tabular}{llll}
\hline
                & \multicolumn{3}{c}{\textsc{Metrics}}                                                   \\ \cline{2-4} 
\textsc{Model-Layer} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{$F_1$} \\ \hline
CodeBERT-0      &                               &                            &                           \\
CodeBERTrand-l  &                               &                            &                           \\ \hline
CodeBERT-l      &                               &                            &                           \\
GraphCodeBERT-l &                               &                            &                           \\
CodeT5-l        &                               &                            &                           \\
CodeBERTa-l     &                               &                            &                           \\
RoBERTa-l       &                               &                            &                           \\ \hline
\end{tabular}
\caption{Result of the probe for each model and Python language. We only report the best layer in each model together with the baselines.}
\end{table}


% test: https://github.com/synercys/annotated_latex_equations
\begin{figure}[htb]
\vspace{2\baselineskip}
\begin{equation}
\vspace{\baselineskip}
            \label{eq:epsilon}
                \pr[\tikzmarknode{x}{\highlight{red}{\mathcal{X}(\cdot)}}\in \tikzmarknode{s}{\highlight{blue}{\mathcal{S}}}] \leq e^\epsilon \cdot \pr[\mathcal{X}(\cdot)\in \mathcal{S}]
\end{equation}
\begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
    % For "X"
    \path (x.north) ++ (0,2em) node[anchor=south east,color=red!67] (scalep){\textbf{system state}};
    \draw [color=red!87](x.north) |- ([xshift=-0.3ex,color=red]scalep.south west);
    % For "S"
    \path (s.south) ++ (0,-1.5em) node[anchor=north west,color=blue!67] (mean){\textbf{$\mathcal{S} \subseteq \mathrm{Range}(\mathcal{X})$}};
    \draw [color=blue!57](s.south) |- ([xshift=-0.3ex,color=blue]mean.south east);
\end{tikzpicture}
\end{figure}


\begin{enumerate}
    \item First of all we have to confirm that our probe is valid. To this end we consider two baselines and compare their performances with the rest of the language models.
    
    \item For all models we study the output embeddings of each one of its layers to see where the AST is encoded.
    
    \item Overall, what model is the best one and discuss some hypothetical reasons why.
\end{enumerate}

\begin{figure}[htb]
$$h_i^l = \tikzmarknode{x}{\highlight{red}{P_\mathcal{S}(h_i^l)}} + \tikzmarknode{y}{\highlight{blue}{P_{\mathcal{S}^ \perp}(h_i^l)}}$$

\begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
    % For "X"
    \path (x.north) ++ (0,1em) node[anchor=south east,color=red!67] (scalep){\textbf{$\in \mathcal{S}$}};
    \draw [color=red!87](x.north) |- ([xshift=-0.3ex,color=red]scalep.south west);
    % For "S"
    \path (y.south) ++ (0,-0.3em) node[anchor=north west,color=blue!67] (mean){\textbf{$\in \mathcal{S}^\perp$}};
    \draw [color=blue!57](y.south) |- ([xshift=-0.3ex,color=blue]mean.south east);
\end{tikzpicture}
\end{figure}



\begin{figure*}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_python.pdf}
         \caption{Python}

     \end{subfigure}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_javascript.pdf}
         \caption{JavaScript}

     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_go.pdf}
         \caption{Go}

     \end{subfigure}
        \caption{Result of the probe for each model, language and layer. The $x-$axis represents the layer number and the $y-$axis shows the $F_1$ score.}
        \label{fig:layervsf1}
\end{figure*}


\begin{figure*}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_rank_python.pdf}
         \caption{Python}

     \end{subfigure}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_rank_javascript.pdf}
         \caption{JavaScript}

     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/myplot_rank_go.pdf}
         \caption{Go}

     \end{subfigure}
        \caption{Result of the probe for each model and best layer, variying the dimension of the subspace. The $x-$axis represents the dimension/rank and the $y-$axis shows the $F_1$ score.}
        \label{fig:layervsrank}
\end{figure*}
